ParBlockchain: Leveraging Transaction Parallelism in Permissioned Blockchain Systems

Many existing blockchains do not adequately address all the characteristics of distributed system applications and suffer from serious architectural limitations resulting in performance and confidentiality issues. While recent permissioned blockchain systems, have tried to overcome these limitations, their focus has mainly been on workloads with no-contention, i.e., no conflicting transactions. In this paper, we introduce OXII, a new paradigm for permissioned blockchains to support distributed applications that execute concurrently. OXII is designed for workloads with (different degrees of) contention. We then present ParBlockchain, a permissioned blockchain designed specifically in the OXII paradigm. The evaluation of ParBlockchain using a series of benchmarks reveals that its performance in workloads with any degree of contention is better than the state of the art permissioned blockchain systems.

==> graph_exe.tex <==
\begin{figure}[t!]
\begin{minipage}{.23\textwidth}\centering
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={Number of executors},
    ylabel={Throughput [trans/sec]},
    xmin=0, xmax=110,
    ymin=0, ymax=6400,
    xtick={20,40,60,80,100},
    ytick={0,1500,3000,4500,6000},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]
 

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (1,1164)(10,1121)(20,1083)(30,1044)(40,1005)(50,954)(60,912)(70,857)(80,793)(90,744)(100,681)};

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (1,6036)(10,5952)(20,5871)(30,5797)(40,5715)(50,5637)(60,5562)(70,5471)(80,5370)(90,5261)(100,5153)};

\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (1,6036)(10,5952)(20,5871)(30,5797)(40,5715)(50,5637)(60,5562)(70,5471)(80,5370)(90,5261)(100,5153)};

\addlegendentry{OX}
\addlegendentry{XOV}
\addlegendentry{OXII}

 
\end{axis}
\end{tikzpicture}
{\footnotesize (a) Throughput}
\end{minipage}\hfill
\begin{minipage}{.23\textwidth} \centering
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={Number of executors},
    ylabel={Latency [s]},
    xmin=0, xmax=110,
    ymin=0, ymax=4.2,
    xtick={20,40,60,80,100},
    ytick={1,2,3,4},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (1,3.656)(10,3.692)(20,3.721)(30,3.747)(40,3.773)(50,3.812)(60,3.841)(70,3.872)(80,3.910)(90,3.954)(100,3.996)};

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (1,0.074)(10,0.077)(20,0.082)(30,0.088)(40,0.091)(50,0.094)(60,0.097)(70,0.100)(80,0.105)(90,0.111)(100,0.119)};

\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (1,0.074)(10,0.077)(20,0.082)(30,0.088)(40,0.091)(50,0.094)(60,0.097)(70,0.100)(80,0.105)(90,0.111)(100,0.119)};

\addlegendentry{OX}
\addlegendentry{XOV}
\addlegendentry{OXII}

 
\end{axis}
\end{tikzpicture}
{\footnotesize (b) Latency}
\end{minipage}
\caption{Throughput/Latency Measurement by increasing the executors}
  \label{fig:exe}
\end{figure}

==> graph_nonexe.tex <==
\begin{figure}[t!]
\begin{minipage}{.23\textwidth}\centering
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={Number of non-executors},
    ylabel={Throughput [trans/sec]},
    xmin=0, xmax=110,
    ymin=0, ymax=6400,
    xtick={20,40,60,80,100},
    ytick={0,1500,3000,4500,6000},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]
 

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (1,1164)(10,1121)(20,1083)(30,1044)(40,1005)(50,954)(60,912)(70,857)(80,793)(90,744)(100,681)};

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (1,6036)(10,5952)(20,5871)(30,5797)(40,5715)(50,5637)(60,5562)(70,5471)(80,5370)(90,5261)(100,5153)};

\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (1,6036)(10,5952)(20,5871)(30,5797)(40,5715)(50,5637)(60,5562)(70,5471)(80,5370)(90,5261)(100,5153)};

\addlegendentry{OX}
\addlegendentry{XOV}
\addlegendentry{OXII}

 
\end{axis}
\end{tikzpicture}
{\footnotesize (a) Throughput}
\end{minipage}\hfill
\begin{minipage}{.23\textwidth} \centering
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={Number of non-executors},
    ylabel={Latency [s]},
    xmin=0, xmax=110,
    ymin=0, ymax=4.2,
    xtick={20,40,60,80,100},
    ytick={1,2,3,4},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (1,3.656)(10,3.692)(20,3.721)(30,3.747)(40,3.773)(50,3.812)(60,3.841)(70,3.872)(80,3.910)(90,3.954)(100,3.996)};

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (1,0.074)(10,0.077)(20,0.082)(30,0.088)(40,0.091)(50,0.094)(60,0.097)(70,0.100)(80,0.105)(90,0.111)(100,0.119)};

\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (1,0.074)(10,0.077)(20,0.082)(30,0.088)(40,0.091)(50,0.094)(60,0.097)(70,0.100)(80,0.105)(90,0.111)(100,0.119)};

\addlegendentry{OX}
\addlegendentry{XOV}
\addlegendentry{OXII}

 
\end{axis}
\end{tikzpicture}
{\footnotesize (b) Latency}
\end{minipage}
\caption{Throughput/Latency Measurement by increasing the non-executors}
  \label{fig:nonexe}
\end{figure}
